Conformal Prediction via Regression-as-Classification

Conformal prediction (CP) for regression can be challenging, especially when the output distribution is heteroscedastic, multimodal, or skewed. Some of the issues can be addressed by estimating a distribution over the output, but in reality, such approaches can be sensitive to estimation error and yield unstable intervals.~Here, we circumvent the challenges by converting regression to a classification problem and then use CP for classification to obtain CP sets for regression.~To preserve the ordering of the continuous-output space, we design a new loss function and make necessary modifications to the CP classification techniques.~Empirical results on many benchmarks shows that this simple approach gives surprisingly good results on many practical problems.

==> subfiles/kprior.tex <==
\subsection{Extension to K-Prior}
While Stochastic Variational Inference solves the posterior via minimizing the ELBO function, the ELBO function notably does not contain any information about the structure of the minimization problem using the previous solution. However, the Bayesian method for approximating a change in the posterior where a datapoint is changed is more exactly captured via the problem of K-Priors \citep{Khan2021}. Namely, they define a K-Prior as the regulator.
\begin{restatable}{definition}{kprior} 
    \label{def:kprior}
    We can form a prior on parameters $\theta$ parameterized by natural parameters $\lambda$ via $$\mathbb{Q}_{\mathcal{K}}(\theta, \mathcal{X}) \propto \operatorname{exp}(- \mathcal{K}(\theta, \mathcal{X}))\text{,}$$ where
    $$\mathcal{K}(\theta) = \sum_{i \in \mathcal{X}} \mathbb{P}(y_i |x_i, \theta^*) - \mathbb{P}(y_i |x_i, \theta) + D_\theta(\theta, \theta^*)\text{.}$$ Here, $\theta^* $ is the optimal $\theta$ and $\mathcal{X}$ is some collection of indices. Unless otherwise stated, we will assume $\mathcal{X} = [n]$. 
\end{restatable}

From \citet{Khan2021}, they provide a general framework for finding a parameter $\theta$ that solves the minimization problem from \Cref{eq:obj}. They phrase this as the minimization problem

\begin{equation}
\underset{\lambda}{\argmin} \enspace \mathbb{E}_{\mathbb{Q}_z^{\lambda}} [P(z|x_{n+1}, \theta)] + D_{KL}(\mathbb{Q}_z^{\lambda}||\mathbb{Q}_{\mathcal{K}(\cdot, \mathcal{X})}(\theta))\text{.} \label{eq:kpriorobj}
\end{equation}
While this is almost identical to the previous problem, we can use the optimization framework from \citet{Khan2021} to solve this minimization problem. The main empirical benefit of this framework is that we \emph{do not need to use the entire dataset to find approximately good solutions}. We can approximate the minimization problem from \Cref{eq:kpriorobj} using the following approximation. 

\begin{equation}   
\underset{\lambda}{\argmin} \enspace \mathbb{E}_{\mathbb{Q}_z^{\lambda}} [P(z|x_{n+1}, \theta)] + D_{KL}(\mathbb{Q}_z^{\lambda}||\mathbb{Q}_{\mathcal{K}(\cdot, \hat{\mathcal{X}})}(\theta))\text{.} \label{eq:kpriorobjapprox}
\end{equation}
Here, $\hat{\mathcal{X}}$ is some subset $\hat{\mathcal{X}} \subset [n]$. Empirically, we see that solving with some smaller set $\hat{\mathcal{X}}$ yields similar solutions to \Cref{eq:kpriorobj} while saving tremendously on computational time. 

\paragraph{Exchangability} While this method is empirically promising, there is one main caveat to such an improvement: \emph{we lose exchangeability guarantees}. The solution to the problem from \Cref{eq:kpriorobjapprox} notably is not invariant with the permutation of the dataset. Unfortunately, the coverage guarantees from \Cref{lem:coverage} do not hold. It remains to be seen if I can implement ad-hoc exchangeability as in \citet{fong2021conformal}. We will have to see if empirically this holds. 


